Holographic geometry/real-space entanglement correspondence and metric reconstruction

In holography, the boundary entanglement structure is believed to be encoded in the bulk geometry. In this work, we investigate the precise correspondence between the boundary real-space entanglement and the bulk geometry. By the boundary real-space entanglement, we refer to the conditional mutual information (CMI) for two infinitesimal subsystems separated by a distance $l$, and the corresponding bulk geometry is at a radial position $z_*$, namely the turning point of the entanglement wedge for a boundary region with a length scale $l$. In a generic geometry described by a given coordinate system, $z_*$ can be determined locally by $l$, while the exact expression for $z_*(l)$ depends on the gauge choice, reflecting the inherent nonlocality of this seemingly local correspondence. We propose to specify the function $z_*(l)$ as the criterion for a gauge choice, and with the specified gauge function, we verify the exact correspondence between the boundary real-space entanglement and the bulk geometry. Inspired by this correspondence, we propose a new method of bulk metric reconstruction from boundary entanglement data, namely the CMI reconstruction. In this CMI proposal, with the gauge fixed a priori by specifying $z_*(l)$, the bulk metric can be reconstructed from the relation between the bulk geometry and the boundary CMI. The CMI reconstruction method establishes a connection between the differential entropy prescription and Bilson's general algorithm for metric reconstruction.

==> bibtem.tex <==
\begin{thebibliography}{99}
%\cite{Witten:2015aoa}
\bibitem{Witten:2015aoa}
E.~Witten,
%``Three lectures on topological phases of matter,''
Riv. Nuovo Cim. \textbf{39}, no.7, 313-370 (2016)
doi:10.1393/ncr/i2016-10125-3
[arXiv:1510.07698 [cond-mat.mes-hall]].
%144 citations counted in INSPIRE as of 16 Feb 2025
%\cite{Landsteiner:2015lsa}

\bibitem{Thouless1}
J. Kosterlitz, D. Thouless, Long range order and metastability in two dimensional 
solids and superfluids. (Application of dislocation theory), Journal of Physics C: Solid 
State Physics, 5: L124, 1972. 

\bibitem{Thouless2}
J. Kosterlitz, D. Thouless, Ordering, metastability and phase transitions in twodimensional
systems, Joumal of Physics C: Solid State Physics, 6: 1181, 1973.

\bibitem{Haldane}
F. D. M. Haldane, Model for a Quantum Hall Effect without Landau Levels: 
Condensed-Matter Realization of the ``Parity Anomaly”, Phys. Rev. Lett.,61: 2015, 1988.

\bibitem{Landsteiner:2015lsa}
  K.~Landsteiner and Y.~Liu,
{\em The holographic Weyl semi-metal,}
 \doi{10.1016/j.physletb.2015.12.052}{Phys.\ Lett.\ B {\bf 753}, 453 (2016)}
  [\arXiv{1505.04772}{hep-th}].

%\cite{Landsteiner:2015pdh}
\bibitem{Landsteiner:2015pdh}
  K.~Landsteiner, Y.~Liu and Y.~W.~Sun,
{\em Quantum phase transition between a topological and a trivial semimetal from holography,}
 \doi{10.1103/PhysRevLett.116.081602}{Phys.\ Rev.\ Lett.\  {\bf 116}, no. 8, 081602 (2016)}
  [\arXiv{1511.05505}{hep-th}].
  %%CITATION = doi:10.1103/PhysRevLett.116.081602;%%
  %15 citations counted in INSPIRE as of 16 Jun 2018

%\cite{Landsteiner:2016stv}
\bibitem{Landsteiner:2016stv}
K.~Landsteiner, Y.~Liu and Y.~W.~Sun,
%``Odd viscosity in the quantum critical region of a holographic Weyl semimetal,''
Phys. Rev. Lett. \textbf{117}, no.8, 081604 (2016)
doi:10.1103/PhysRevLett.117.081604
[arXiv:1604.01346 [hep-th]].
%47 citations counted in INSPIRE as of 16 Feb 2025


%\cite{Bachas:2020yxv}
\bibitem{Bachas:2020yxv}
C.~Bachas, S.~Chapman, D.~Ge and G.~Policastro,
%``Energy Reflection and Transmission at 2D Holographic Interfaces,''
Phys. Rev. Lett. \textbf{125} (2020) no.23, 231602
doi:10.1103/PhysRevLett.125.231602
[arXiv:2006.11333 [hep-th]].

%\cite{Simidzija:2020ukv}
\bibitem{Simidzija:2020ukv}
P.~Simidzija and M.~Van Raamsdonk,
%``Holo-ween,''
JHEP \textbf{12} (2020), 028
doi:10.1007/JHEP12(2020)028
[arXiv:2006.13943 [hep-th]].


%\cite{Liu:2024oxg}
\bibitem{Liu:2024oxg}
Y.~Liu, H.~D.~Lyu and C.~Y.~Wang,
%``On AdS$_{3}$/ICFT$_{2}$ with a dynamical scalar field located on the brane,''
JHEP \textbf{10} (2024), 001
doi:10.1007/JHEP10(2024)001
[arXiv:2403.20102 [hep-th]].


%\cite{Liu:2025gle}
\bibitem{Liu:2025gle}
Y.~Liu, C.~Y.~Wang and Y.~J.~Zeng,
%``Energy transport in holographic non-conformal interfaces,''
[arXiv:2503.20399 [hep-th]].

%\cite{Grignani:2016wyz}
\bibitem{Grignani:2016wyz}
G.~Grignani, A.~Marini, F.~Pena-Benitez and S.~Speziali,
%``AC conductivity for a holographic Weyl Semimetal,''
JHEP \textbf{03}, 125 (2017)
doi:10.1007/JHEP03(2017)125
[arXiv:1612.00486 [cond-mat.str-el]].
%23 citations counted in INSPIRE as of 16 Feb 2025


%\cite{Copetti:2016ewq}
\bibitem{Copetti:2016ewq}
C.~Copetti, J.~Fern\'andez-Pend\'as and K.~Landsteiner,
%``Axial Hall effect and universality of holographic Weyl semi-metals,''
JHEP \textbf{02}, 138 (2017)
doi:10.1007/JHEP02(2017)138
[arXiv:1611.08125 [hep-th]].
%34 citations counted in INSPIRE as of 16 Feb 2025


%\cite{Bu:2018vcp}
\bibitem{Bu:2018vcp}
Y.~Bu, R.~G.~Cai, Q.~Yang and Y.~L.~Zhang,
%``Holographic Charged Fluid with Chiral Electric Separation Effect,''
JHEP \textbf{09}, 083 (2018)
doi:10.1007/JHEP09(2018)083
[arXiv:1803.08389 [hep-th]].
%8 citations counted in INSPIRE as of 16 Feb 2025


%\cite{Ji:2019pxx}
\bibitem{Ji:2019pxx}
X.~Ji, Y.~Liu and X.~M.~Wu,
%``Chiral vortical conductivity across a topological phase transition from holography,''
Phys. Rev. D \textbf{100}, no.12, 126013 (2019)
doi:10.1103/PhysRevD.100.126013
[arXiv:1904.08058 [hep-th]].
%12 citations counted in INSPIRE as of 16 Feb 2025 

%\cite{Landsteiner:2019kxb}
\bibitem{Landsteiner:2019kxb}
K.~Landsteiner, Y.~Liu and Y.~W.~Sun,
%``Holographic topological semimetals,''
Sci. China Phys. Mech. Astron. \textbf{63}, no.5, 250001 (2020)
doi:10.1007/s11433-019-1477-7
[arXiv:1911.07978 [hep-th]].
%32 citations counted in INSPIRE as of 16 Feb 2025

\bibitem{tknn}
Thouless, D. J., Kohmoto, M., Nightingale, M. P., den Nijs, M. (1982).
Quantized Hall Conductance in a Two-Dimensional Periodic Potential.
Physical Review Letters, 49(6), 405-408.

\bibitem{km1}
Kane, C. L., Mele, E. J. (2005).
Quantum Spin Hall Effect in Graphene.
Physical Review Letters, 95(22), 226801.


\bibitem{moore}
Moore, J. E., Balents, L. (2007).
Topological invariants of time-reversal-invariant band structures.
Physical Review B, 75(12), 121306.

\bibitem{km2}
Fu, L., Kane, C. L., Mele, E. J. (2007).
Topological Insulators in Three Dimensions.
Physical Review Letters, 98(10), 106803.


\bibitem{qi1}
Qi, X.-L., Hughes, T. L., Zhang, S.-C. (2008).
Topological Field Theory of Time-Reversal Invariant Insulators.
Physical Review B, 78(19), 195424.


\bibitem{Armitage}
Armitage, Mele , Vishwanath (2018)
Rev. Mod. Phys. 90, 015001.


\bibitem{Hasan}
Hasan, Kane (2010)
Rev. Mod. Phys. 82, 3045.


\bibitem{Ninomiya}
H.~B.~Nielsen and M.~Ninomiya,
{}{\em Adler-Bell-Jackiw anomaly and Weyl fermions in crystal,}{}
%Phys. Lett. B \textbf{130}, 389-396 (1983)
\doi{10.1016/0370-2693(83)91529-0}{Phys. Lett. B \textbf{130}, 389-396 (1983)}.



\bibitem{wan}
Wan, Turner, Vishwanath, Savrasov (2011)
Phys. Rev. B 83, 205101.


\bibitem{pan}
Z. Wang, X. Cheng, B. Wang, et al., Realization of an ideal Weyl semimetal band in a 
quantum gas with 3D spin-orbit coupling, Science, 372: 271, 2021.


\bibitem{Ji:2021aan}
X.~Ji, Y.~Liu, Y.~W.~Sun and Y.~L.~Zhang,
%``A Weyl-Z$_{2}$ semimetal from holography,''
JHEP \textbf{12}, 066 (2021)
doi:10.1007/JHEP12(2021)066
[arXiv:2109.05993 [hep-th]].

\bibitem{witten}
E. Witten, Anti de sitter space and holography, Adv. Theor. Math. Phys., 2: 253, 1998. 


\bibitem{gubser}
S. Gubser, I. Klebanov, A. Polyakov, Gauge theory correlators from noncritical string 
theory, Phys. Lett. B, 428:105, 1998. 


\bibitem{wang-prx1}
  Z.~Wang and S.~C.~Zhang,
{\em Topological Invariants and Ground-State Wave Functions of Topological Insulators on a Torus,}
\doi{10.1103/PhysRevX.4.011006}{Phys.\ Rev.\ X {\bf 4}, no. 1, 011006 (2014)}
[\arXiv{1308.4900}{cond-mat.str-el}].


\bibitem{wang-prx2}
Z.~Wang and S.~C.~Zhang, {\em Simplified topological invariants for interacting insulators,}
\doi{10.1103/PhysRevX.2.031008}{Phys.\ Rev.\ X {\bf 2}, 031008 (2012)}.


%\cite{Wang:2012ig}
\bibitem{Wang:2012ig}
  Z.~Wang and B.~Yan,
{\em Topological Hamiltonian as an Exact Tool for Topological Invariants,}
%  J.\ Phys.\ : Condens.\ Matter {\bf 25}, 155601 (2013)
  \doi{10.1088/0953-8984/25/15/155601}{J.\ Phys.\ : Condens.\ Matter {\bf 25}, 155601 (2013)}
  [\arXiv{1207.7341}{cond-mat.str-el}].
  %%CITATION = doi:10.1088/0953-8984/25/15/155601;%%

%\cite{Zaanen:2015oix}
\bibitem{Zaanen:2015oix}
  J.~Zaanen, Y.~W.~Sun, Y.~Liu and K.~Schalm,
 \href{http://www.cambridge.org/de/academic/subjects/physics/condensed-matter-physics-nanoscience-and-mesoscopic-physics/holographic-duality-condensed-matter-physics?format=HB#AlwhgydkVTSFfv7H.97}{\em Holographic Duality in Condensed Matter Physics,}  Cambridge University Press, 2015.
  %%CITATION = INSPIRE-1384852;%%
  
  
\bibitem{book}
M.~Ammon and J.~Erdmenger,
\href{http://www.cambridge.org/de/academic/subjects/physics/theoretical-physics-and-mathematical-physics/gaugegravity-duality-foundations-and-applications#xOzmEecLSr4ZJFIH.97}{\em Gauge/gravity duality: Foundations and applications},
Cambridge University Press, 2015.
%\cite{Hartnoll:2016apf}


\bibitem{review}
  S.~A.~Hartnoll, A.~Lucas and S.~Sachdev,
{\em Holographic quantum matter,}
[\arXiv{1612.07324}{hep-th}].
  %%CITATION = ARXIV:1612.07324;%%



%\cite{Bahamondes:2024zsm}
\bibitem{Bahamondes:2024zsm}
S.~Bahamondes, I.~Salazar Landea and R.~Soto-Garrido,
%``Holographic description of an anisotropic Dirac semimetal,''
JHEP \textbf{09}, 080 (2024)
doi:10.1007/JHEP09(2024)080
[arXiv:2406.00156 [hep-th]].
%1 citations counted in INSPIRE as of 17 Feb 2025


\bibitem{Liu:2018bye}
Y.~Liu and Y.~W.~Sun,
{}{\em Topological nodal line semimetals in holography,}{}
%JHEP \textbf{12} (2018), 072.
\doi{10.1007/JHEP12(2018)072}{JHEP \textbf{12} (2018), 072}
[\arXiv{1801.09357}{hep-th}].
%9 citations counted in INSPIRE as of 15 Jun 2020

%\cite{Liu:2020ymx}
\bibitem{Liu:2020ymx}
Y.~Liu and X.~M.~Wu,
{\em An improved holographic nodal line semimetal,}
[\arXiv{2012.12602}{hep-th}].


%\cite{Chu:2024dti}
\bibitem{Chu:2024dti}
H.~Chu, X.~Ji and Y.~W.~Sun,
%``Coexistence of topological semimetal states in holography,''
JHEP \textbf{05}, 166 (2024)
doi:10.1007/JHEP05(2024)166
[arXiv:2403.02669 [hep-th]].
%2 citations counted in INSPIRE as of 17 Feb 2025


%\cite{Liu:2018djq}
\bibitem{Liu:2018djq}
Y.~Liu and Y.~W.~Sun,
%``Topological invariants for holographic semimetals,''
JHEP \textbf{10}, 189 (2018)
doi:10.1007/JHEP10(2018)189
[arXiv:1809.00513 [hep-th]].
%27 citations counted in INSPIRE as of 07 Feb 2025
%\cite{Ji:2021aan}

%\cite{Song:2019asj}
\bibitem{Song:2019asj}
G.~Song, J.~Rong and S.~J.~Sin,
%``Stability of topology in interacting Weyl semi-metal and topological dipole in holography,''
JHEP \textbf{10}, 109 (2019)
doi:10.1007/JHEP10(2019)109
[arXiv:1904.09349 [hep-th]].
%14 citations counted in INSPIRE as of 17 Feb 2025

%\cite{Ji:2023rua}
\bibitem{Ji:2023rua}
X.~Ji and Y.~W.~Sun,
%``Topological phase transitions of semimetal states in effective field theory models,''
Eur. Phys. J. Plus \textbf{139}, 485 (2024)
doi:10.1140/epjp/s13360-024-05291-z
[arXiv:2302.07421 [cond-mat.mes-hall]].
%2 citations counted in INSPIRE as of 17 Feb 2025
%\cite{Grushin:2012mt}

\bibitem{Grushin:2012mt}
  A.~G.~Grushin,
 {\em Consequences of a condensed matter realization of Lorentz violating QED in Weyl semi-metals,}
 % Phys.\ Rev.\ D {\bf 86}, 045001 (2012)
  \doi{10.1103/PhysRevD.86.045001}{Phys.\ Rev.\ D {\bf 86}, 045001 (2012)},
  [\arXiv{1205.3722}{hep-th}].
  %%CITATION = doi:10.1103/PhysRevD.86.045001;%%

 %\cite{Grushin:2019uuu}
 
\bibitem{Grushin:2019uuu}
  A.~G.~Grushin,
{\em Common and not so common high-energy theory methods for condensed matter physics,}
  %doi:10.1007/978-3-319-76388-0_6
 \arXiv{1909.02983}{cond-mat.mes-hall}.
 
%\cite{Liu:2009dm}
\bibitem{Liu:2009dm}
H.~Liu, J.~McGreevy and D.~Vegh,
%``Non-Fermi liquids from holography,''
Phys. Rev. D \textbf{83}, 065029 (2011)
doi:10.1103/PhysRevD.83.065029
[arXiv:0903.2477 [hep-th]].
%554 citations counted in INSPIRE as of 03 Mar 2025 

%\cite{Cubrovic:2009ye}
\bibitem{Cubrovic:2009ye}
M.~Cubrovic, J.~Zaanen and K.~Schalm,
%``String Theory, Quantum Phase Transitions and the Emergent Fermi-Liquid,''
Science \textbf{325}, 439-444 (2009)
doi:10.1126/science.1174962
[arXiv:0904.1993 [hep-th]].
%449 citations counted in INSPIRE as of 03 Mar 2025

%\cite{Plantz:2018tqf}
\bibitem{Plantz:2018tqf}
N.~W.~M.~Plantz, F.~Garc\'\i{}a Fl\'orez and H.~T.~C.~Stoof,
%``Massive Dirac fermions from holography,''
JHEP \textbf{04}, 123 (2018)
doi:10.1007/JHEP04(2018)123
[arXiv:1802.04191 [hep-th]].
%10 citations counted in INSPIRE as of 03 Mar 2025

%\cite{Iqbal:2011in}
\bibitem{Iqbal:2011in}
N.~Iqbal, H.~Liu and M.~Mezei,
%``Semi-local quantum liquids,''
JHEP \textbf{04}, 086 (2012)
doi:10.1007/JHEP04(2012)086
[arXiv:1105.4621 [hep-th]].
%139 citations counted in INSPIRE as of 03 Mar 2025

%\cite{Hartnoll:2010gu}
\bibitem{Hartnoll:2010gu}
S.~A.~Hartnoll and A.~Tavanfar,
%``Electron stars for holographic metallic criticality,''
Phys. Rev. D \textbf{83}, 046003 (2011)
doi:10.1103/PhysRevD.83.046003
[arXiv:1008.2828 [hep-th]].
%172 citations counted in INSPIRE as of 03 Mar 2025

%\cite{Hartnoll:2011dm}
\bibitem{Hartnoll:2011dm}
S.~A.~Hartnoll, D.~M.~Hofman and D.~Vegh,
%``Stellar spectroscopy: Fermions and holographic Lifshitz criticality,''
JHEP \textbf{08}, 096 (2011)
doi:10.1007/JHEP08(2011)096
[arXiv:1105.3197 [hep-th]].
%96 citations counted in INSPIRE as of 03 Mar 2025

%\cite{Cubrovic:2011xm}
\bibitem{Cubrovic:2011xm}
M.~Cubrovic, Y.~Liu, K.~Schalm, Y.~W.~Sun and J.~Zaanen,
%``Spectral probes of the holographic Fermi groundstate: dialing between the electron star and AdS Dirac hair,''
Phys. Rev. D \textbf{84}, 086002 (2011)
doi:10.1103/PhysRevD.84.086002
[arXiv:1106.1798 [hep-th]].
%42 citations counted in INSPIRE as of 03 Mar 2025

%\cite{Liu:2014mva}
\bibitem{Liu:2014mva}
Y.~Liu, K.~Schalm, Y.~W.~Sun and J.~Zaanen,
%``BCS instabilities of electron stars to holographic superconductors,''
JHEP \textbf{05}, 122 (2014)
doi:10.1007/JHEP05(2014)122
[arXiv:1404.0571 [hep-th]].
%5 citations counted in INSPIRE as of 03 Mar 2025

\bibitem{future}
X. Chen,  X. Ji and Y. W. Sun, working in progress.

\bibitem{im1}
X. Ji, H. Lu, Z. Zhu, and G. Su, ``Effect of the screened Coulomb disorder on magnetotransport
in Weyl semimetals", J. Appl. Phys. 123: 203901, 2018.

\bibitem{im2}
C. Xu, H. Yu, M. Zhou and X. Ji, ``Induced magneto-conductivity in a two-nodes Weyl 
semimetal under Gaussian random disorder", 
Chin. Phys. B, 33(9): 097502, 2024.


\bibitem{Symplectic}
Feng, Kang, and  M.~Qin,
{}{\em Symplectic Geometric Algorithms for Hamiltonian Systems,} Springer (2010).


\bibitem{Chern-Weil}
Zhang, Weiping,
{}{\em Lectures on Chern-Weil theory and Witten deformations,}{} World Scientific Publishing Co.inc.river Edge Nj 4(2002):132.


bibitem{Spin}
Lawson, H.~Blaine , and  M.~ L.~ Michelsohn,
{}{\em Spin geometry,}
10.1515/9781400883912(1990).
\end{thebibliography}
